Sci-MMR: Benchmarking Multi-Step Evidence-Grounded Scientific Reasoning in Multimodal Agents

Autonomous research agents are increasingly expected to search the literature, analyze experimental evidence, and generate scientific hypotheses. These capabilities require multi-step evidence grounded reasoning that progressively acquires, integrates, and verifies evidence before reaching a conclusion. Existing multimodal benchmarks, however, largely evaluate final-answer accuracy, leaving open whether predictions are actually supported by traceable scientific evidence. We introduce Sci-MMR, a benchmark for multi-step evidence-grounded scientific reasoning built on structured argument graphs linking scientific claims, citation-grounded knowledge, visual evidence, and supporting regions. Sci-MMR comprises 235 multi-hop reasoning tasks spanning four scientific disciplines, with an average of nine figure panels per task. Evaluating eight frontier multimodal models, we find that answer accuracy consistently exceeds complete-evidence recovery rate by more than 20%, revealing a substantial gap that answer-only evaluation is structurally unable to capture. Through controlled interventions, we identify two fundamental bottlenecks. First, evidence acquisition: models struggle to extract complete structured evidence from scientific figures, accounting for 57.2% of failures. While cropping tools yield modest gains (+4.5 points), providing gold evidence improves accuracy by up to 37.0 points, indicating difficulty in assembling complete multi-region evidence. Second, evidence integration: models struggle to translate available evidence into correct conclusions, accounting for 31.8% of failures, while even with gold evidence the strongest model achieves only 69.1% accuracy on the hardest tasks. These findings indicate that current answer-centric benchmarks substantially overestimate the evidence-grounded reasoning capabilities of multimodal research agents

==> Figures/supp_rq1_stratified_accuracy.tex <==
% Generated by build_supplementary_material.py; do not edit values manually.
\begin{table*}[!t]
\centering
\scriptsize
\setlength{\tabcolsep}{5.0pt}
\begin{tabular}{lrrrrrrr}
\toprule
Model & Bio. & Chem. & Comp. & Phys. & Hard & Med. & Easy \\
\midrule
GPT-5.5 & 54.0 & 76.5 & 73.0 & 68.2 & 29.6 & 81.5 & 96.8 \\
Claude Opus 4.8 & 48.0 & 76.5 & 61.9 & 45.5 & 11.1 & 66.3 & 95.2 \\
Kimi K2.7 & 46.0 & 55.9 & 58.7 & 45.5 & 11.1 & 56.5 & 93.5 \\
Gemini 3.1 Pro & 46.0 & 61.8 & 49.2 & 48.9 & 9.9 & 58.7 & 90.3 \\
MiniMax-M3 & 46.0 & 58.8 & 46.0 & 39.8 & 4.9 & 48.9 & 93.5 \\
GLM-5V Turbo & 46.0 & 50.0 & 36.5 & 38.6 & 8.6 & 41.3 & 83.9 \\
Qwen3.7 Plus & 40.0 & 41.2 & 33.3 & 21.6 & 4.9 & 28.3 & 71.0 \\
Intern-S2 & 30.0 & 32.4 & 23.8 & 25.0 & 4.9 & 16.3 & 71.0 \\
\midrule
\textbf{Pooled} & 44.5 & 56.6 & 47.8 & 41.6 & 10.6 & 49.7 & 86.9 \\
\bottomrule
\end{tabular}
\caption{Direct Visual Reasoning accuracy (\%) by scientific discipline and difficulty defined from Direct Visual Reasoning.}
\label{tab:supp_rq1_stratified}
\end{table*}

